Testing side-channel security of cryptographic implementations against future microarchitectures

How will future microarchitectures impact the security of existing cryptographic implementations? As we cannot keep reducing the size of transistors, chip vendors have started developing new microarchitectural optimizations to speed up computation. A recent study (Sanchez Vicarte et al., ISCA 2021) suggests that these optimizations might open the Pandora's box of microarchitectural attacks. However, there is little guidance on how to evaluate the security impact of future optimization proposals. To help chip vendors explore the impact of microarchitectural optimizations on cryptographic implementations, we develop (i) an expressive domain-specific language, called LmSpec, that allows them to specify the leakage model for the given optimization and (ii) a testing framework, called LmTest, to automatically detect leaks under the specified leakage model within the given implementation. Using this framework, we conduct an empirical study of 18 proposed microarchitectural optimizations on 25 implementations of eight cryptographic primitives in five popular libraries. We find that every implementation would contain secret-dependent leaks, sometimes sufficient to recover a victim's secret key, if these optimizations were realized. Ironically, some leaks are possible only because of coding idioms used to prevent leaks under the standard constant-time model.

==> Makefile <==
PAPER_SRC=pandora.tex
PAPER_OUT=pandora.pdf
LATEX_OUT:=.

BUILTINS := builtins
EXTENSIONS := extensions

# Either specify USE_LATEXRUN=1 when calling the makefile or
# uncomment the next line if you prefer the LATEXRUN python tool
USE_LATEXRUN:=1

USE_SHELLESCAPE:=-shell-escape

LATEXRUN := $(BUILTINS)/latexrun.py --latex-args=$(USE_SHELLESCAPE)\ --synctex=1 -O $(LATEX_OUT) -o $(LATEX_OUT)/_build.pdf
LATEXMK := latexmk -pdf $(USE_SHELLESCAPE) -outdir=$(LATEX_OUT)

# Require VERBOSE=1 to print all the commands run
ifndef VERBOSE
.SILENT:
endif

# Always build because the latex tool does fancy dependency analysis for us
.PHONY: build
build:
	rm -f paper.pdf
ifdef USE_LATEXRUN
		$(LATEXRUN) $(PAPER_SRC)
		if ! cmp --quiet $(LATEX_OUT)/_build.pdf $(PAPER_OUT); then cp $(LATEX_OUT)/_build.pdf $(PAPER_OUT); fi
else
		$(LATEXMK) $(PAPER_SRC)
		cp $(LATEX_OUT)/$(patsubst %.tex,%.pdf,$(PAPER_SRC)) $(PAPER_OUT)
endif

# Allow `make` to just build the paper
.DEFAULT_GOAL := build

.PHONY: clean
clean:
	rm -f pandora.pdf
ifdef USE_LATEXRUN
		$(LATEXRUN) --clean-all
else
		$(LATEXMK) -C
endif
	rm -f *.aux *.bbl *.dvi

# Useful for editor integrations. Will output the full build log
# rather than the just the abbreviated latexrun output.
# You will need to use the --ignore-errors flag though
.PHONY: with-log
with-log: build
	cat $(LATEX_OUT)/$(basename $(notdir $(PAPER_SRC))).log

# Spellchecking
# ----------------------------

# list all unknown-words
.PHONY: unknown-words
unknown-words: build
	for file in `$(BUILTINS)/ltxdeps.sh`; do \
		words="$$(aspell --home-dir=./ list -t < "$$file")"; \
		if [ $$? -eq 0 ]; then \
			grep --color=auto -Hn -Ew "$$(echo $$words | sed -e 's/ /|/g')" $$file; \
		fi \
	done

# Run aspell interactively on all tex files that were built into PAPER_OUT
.PHONY: aspell
aspell: build
	for file in `$(BUILTINS)/ltxdeps.sh`; do \
		read -p "Press ENTER to check $$file:"; \
		aspell --home-dir=./ check -t $$file; \
	done



==> background.tex <==
\section{Background}
\label{sec:bg}
\label{sec:background}

\newcommand{\prog}{\ensuremath{\mathit{Prog}}\xspace}
\newcommand{\con}[2]{\ensuremath{\llbracket{\cdot}\rrbracket^{#2}_{#1}}\xspace}
\newcommand{\pol}{\ensuremath{\mathit{Pol}}\xspace}
\newcommand{\public}{\ensuremath{\mathit{pub}}\xspace}
\newcommand{\secret}{\ensuremath{\mathit{sec}}\xspace}
\newcommand{\exec}[3]{\ensuremath{\llbracket{#1}\rrbracket^{#3}_{#2}}}
\newcommand{\LM}{\ensuremath{L}\xspace}
\newcommand{\XM}{\ensuremath{X}\xspace}


Side-channels are a main concern for security-sensitive programs.  In
particular, side-channel attacks are a major issue for cryptographic
implementations, which must make provisions to ensure that sensitive
data, such as encryption keys, is not leaked. Typically, cryptographic
implementations follow the constant-time (CT) discipline, and ensure
that programs control flow and memory accesses do not depend on
secrets. The CT discipline provides provable security guarantees
against cache-based timing attacks. However, these guarantees are
limited to a classic model of execution and do not consider executions
where instructions execute speculatively or out-of-order. In addition,
the CT discipline implicitly limits the ability of the adversary to
observe cache hits and cache misses. However, modern CPUs aggressively
optimize for performance. These optimizations trigger many forms of
leakage that are not considered by the CT discipline. For instance,
they may leak if a value is within a certain range (e.g. large or
small) or exact to a specific value (e.g.\, zero), or if it is already
stored in memory or has been computed before. \citet{pandorasbox}
surveys and discusses security implications of optimizations that leak
beyond the CT model. In summary, the CT programming discipline assumes
a restricted execution model, and a restricted leakage model. As a
consequence, CT programs can leak and be vulnerable to practical
side-channel attacks.

The limitations of the CT programming discipline can be addressed by
using richer leakage and execution models. While this can be done on a
case-by-case basis, a principled approach is required for building the
necessary tooling to analyze software at scale and across a variety of
attacker models.  Hardware-software contracts provide a principled
foundation for such tooling. Informally, a hardware-software contract
defines a leakage model, which specifies what an attacker can observe
during execution, and an execution mode, which specifies how programs
are executed. Both leakage and execution models are executable, and
define an instrumented adversarial semantics. This semantics collects
leakage traces for all possible executions of a program, and serves as
a basis for reasoning about program leakage. Specifically, a program
is non-interfering with respect to an equivalence relation on states
if pairs of executions starting from equivalent states yield equal
leakage traces. This notion of non-interference subsumes the
constant-time policy, the speculative constant-time policy, and their
elaboration. Similar to these policies, the notion of contract
non-interference can be used by developers to inform the
development of their code, with the guarantee that programs which
are non-interfering w.r.t.\, some contract will execute securely on
hardware that does satisfy the contract.

Contract non-interference also provides a framework in which to
contextualize side-channel attacks, such as Spectre~\cite{spectre} or
Augury~\cite{augury}.  When understood in the context of this paper,
these attacks can be construed as successful exploits of violations of
the $\mathcal{C}$-NI policy for a hardware-software contract
$\mathcal{C}$ that defines the attacker's capability.



















